SAR3D: Autoregressive 3D Object Generation and Understanding via Multi-scale 3D VQVAE

Autoregressive models have demonstrated remarkable success across various fields, from large language models (LLMs) to large multimodal models (LMMs) and 2D content generation, moving closer to artificial general intelligence (AGI). Despite these advances, applying autoregressive approaches to 3D object generation and understanding remains largely unexplored. This paper introduces Scale AutoRegressive 3D (SAR3D), a novel framework that leverages a multi-scale 3D vector-quantized variational autoencoder (VQVAE) to tokenize 3D objects for efficient autoregressive generation and detailed understanding. By predicting the next scale in a multi-scale latent representation instead of the next single token, SAR3D reduces generation time significantly, achieving fast 3D object generation in just 0.82 seconds on an A6000 GPU. Additionally, given the tokens enriched with hierarchical 3D-aware information, we finetune a pretrained LLM on them, enabling multimodal comprehension of 3D content. Our experiments show that SAR3D surpasses current 3D generation methods in both speed and quality and allows LLMs to interpret and caption 3D models comprehensively.

==> tables/quant-3dgen-withGA.tex <==
% \textbf{Ours}         & \cellcolor{tablered}{89.06} & \cellcolor{orange}{24.21}  & \cellcolor{orange}{0.76}  & \cellcolor{tablered}{65.17} & \cellcolor{tablered}{8.72}  & \cellcolor{tablered}{3.22}  & \cellcolor{yellow}{59.50} & \cellcolor{tablered}{15.48} \\


\begin{table*}[t]
\vspace{-2mm}
\centering
\small
\caption{
\textbf{Quantitative Evaluation of Image-conditioned 3D Generation.} We evaluate the quality of both 2D rendering and 3D shapes. As shown below, the proposed method demonstrates strong performance across all metrics. 
%Although multi-view images-to-3D approaches like LGM achieves better performance on the FID/KID metrics, they fall short on more advanced image quality assessment metrics such as MUSIQ and performs significantly worse in 3D shape quality. 
Although LGM, a multi-view images-to-3D approach, achieves slightly better performance on FID, it falls short on more advanced image quality assessment metrics such as MUSIQ and has significantly worse 3D shape quality.
For multi-view to 3D methods, we also include the number of input views (V=$\#$). The latency time is all profiled on Tesla V100 architecture.
}

% \vspace{-0.2cm}
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{l@{\hspace{16mm}}cccccc}
\toprule
Method&FID$\downarrow$&KID(\%)$\downarrow$&MUSIQ$\uparrow$ &COV(\%)$\uparrow$&MMD(\textperthousand)$\downarrow$ & Latency-V100 (s) $\downarrow$   \\
\toprule
Splatter-Image                   & 48.80  & 3.65  & 30.33 & 37.66 & {30.69} & \cellcolor{tablered}{0.83} \\
OpenLRM                        & 38.41  & 1.87  & 45.46  & 39.33 & 29.08 & 7.21 \\
\midrule
One-2-3-45 (V=12)                     & 88.39  & 6.34 & 59.02  & 33.33 & 35.09 & 59.23 \\
Lara (V=4)                          & 43.74  & 1.95  & 39.37  & 39.33 & 28.84 & 11.93 \\
CRM (V=6)                           & 45.53  & 1.93  & \cellcolor{yellow}{64.10}   & 38.83 & 28.91 & 22.10 \\
LGM (V=4)        & \cellcolor{tablered}{19.93}  & \cellcolor{orange}{0.55}  & 54.78   & 50.83 & 22.06 & 3.87 \\
\midrule
Shap-E                        & 138.53 & 11.95 & 31.51   & \cellcolor{orange}{61.33} & \cellcolor{yellow}19.17 & 9.54 \\
GaussianAnything                        & 24.21 & 0.76 & 65.17   & {59.50} & 15.48 & 9.54 \\
LN3Diff & 29.08  & 0.89  & 50.39 & 55.17 & 19.94 & 7.51 \\
% \midrule
\textbf{\nickname{}}-NeRF         & \cellcolor{orange}{22.55}  & \cellcolor{tablered}{0.42}  & \cellcolor{orange}{65.77} & \cellcolor{tablered}{74.17} & \cellcolor{tablered}{13.63} & \cellcolor{orange}{1.64} \\
\textbf{\nickname{}}-Flexicubes         & \cellcolor{yellow}{27.30}  & \cellcolor{yellow}{0.63}  & \cellcolor{tablered}{67.24} & \cellcolor{yellow}{71.50} & \cellcolor{orange}{15.25} & \cellcolor{yellow}{2.92} \\
% \textbf{\nickname{}}-Flexicubes         & \cellcolor{yellow}{27.30}  & \cellcolor{yellow}{0.63}  & \cellcolor{orange}{65.17} & \cellcolor{yellow}{59.50} & \cellcolor{orange}{15.48} & \cellcolor{yellow}{2.92} \\
% \textbf{\nickname{}}-NeRF         & \cellcolor{orange}{22.55}  & \cellcolor{tablered}{0.42}  & \cellcolor{tablered}{67.24} & \cellcolor{tablered}{71.50} & \cellcolor{tablered}{15.24} & 0.82 \\
% \textbf{\nickname{}}-Flexicubes         & \cellcolor{yellow}{27.30}  & \cellcolor{yellow}{0.63}  & \cellcolor{orange}{65.17} & \cellcolor{yellow}{59.50} & \cellcolor{orange}{15.48} & 1.46 \\
\bottomrule
\end{tabular}
}
% \end{adjustbox}
\label{tab:3d-quant-metrics}
\end{table*}

% \textbf{GaussianAnything}  & \cellcolor{orange}{24.21}  & \cellcolor{orange}{0.76}  & \cellcolor{tablered}{65.17} & \cellcolor{tablered}{8.72}  & \cellcolor{tablered}{3.22}  & \cellcolor{yellow}{59.50} & \cellcolor{tablered}{15.48} \\

